Learning Continuous Cost-to-Go Functions for Non-holonomic Systems

This paper presents a supervised learning method to generate continuous cost-to-go functions of non-holonomic systems directly from the workspace description. Supervision from informative examples reduces training time and improves network performance. The manifold representing the optimal trajectories of a non-holonomic system has high-curvature regions which can not be efficiently captured with uniform sampling. To address this challenge, we present an adaptive sampling method which makes use of sampling-based planners along with local, closed-form solutions to generate training samples. The cost-to-go function over a specific workspace is represented as a neural network whose weights are generated by a second, higher order network. The networks are trained in an end-to-end fashion. In our previous work, this architecture was shown to successfully learn to generate the cost-to-go functions of holonomic systems using uniform sampling. In this work, we show that uniform sampling fails for non-holonomic systems. However, with the proposed adaptive sampling methodology, our network can generate near-optimal trajectories for non-holonomic systems while avoiding obstacles. Experiments show that our method is two orders of magnitude faster compared to traditional approaches in cluttered environments.

==> inline_todonotes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following makes inline todonotes behave nicely
\usepackage{todonotes,varwidth}
\makeatletter
\tikzstyle{diaanotestyle} = [
    draw=\@todonotes@currentbordercolor,
    fill=\@todonotes@currentbackgroundcolor,
    line width=0.5pt,
    inner sep = 0.8 ex,
    rounded corners=4pt,align=left,
   ]

\renewcommand{\@todonotes@drawInlineNote}{%
        {\begin{tikzpicture}[remember picture,baseline={(0,0)}]%
            \draw node[diaanotestyle,font=\@todonotes@sizecommand,anchor=base west]{%
               \begin{varwidth}[t]{5cm}
                \if@todonotes@authorgiven%
                    {\@todonotes@sizecommand \@todonotes@author:\,\@todonotes@text}%
                \else%
                    {\@todonotes@sizecommand \@todonotes@text}%
                \fi
                \end{varwidth}};%
            \end{tikzpicture}}%
       }%
\makeatother   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> old-intro.tex <==
\section{The Old Introduction}


%Wiki: Because the final state of the system depends on the intermediate values of its trajectory through parameter space, the system cannot be represented by a conservative potential function as can,

        
    % \item Constraints in robotics (manipulator, car-like robot, etc)
    %     \begin{itemize}
    %         \item There is no known analytical representation for many types of constraint manifolds 
    %         \item Representing the manifold by exhaustive sampling  but expensive
    %         \item Performance is significantly degraded due to constraints
    %     \end{itemize}
    
    % \item Difficulty of nonholonomic system
    %     \begin{itemize}
    %         \item Many mobile robots and vehicles with nonholonomic constraints
    %         \item Two feasible configurations might not be connected due to kinematic constraint
    %         \item Make planning problems difficult such as sampling based planning and  Search based planning approaches (A* and Dijkstra)
    %         \item Need dense sampling or predefined primitives
    %     \end{itemize}
        

Many motion planning algorithms have been researched for robotic systems to move from one configuration to another configuration autonomously such as search based approaches and sampling based approaches. \cite{bonet2001planning,maximARA,lavalle2001randomized}. In order to compute a sequence of valid control inputs for the desired goal configuration, motion planning considers many constraints such as geometric relations with other objects such as obstacles. Nonholonomic constraint is a nonintegrable kinematic constraint including derivative of states, which is inherently imposed by the system's kinematics. Since the nonholonomic constraint limits the system to move states in any directions, motion planning for nonholonomic systems is more difficult compared to motion planning for systems without constraints. Since there is no analytical method for nonholonomic systems in cluttered environments, many traditional planners search the sequence of valid control inputs based on predefined primitives or exhaustive sampling of control inputs \cite{paden2016survey}. These approaches necessitate expensive computation to achieve the desired configuration. 
     
In this paper, we  develop an approach of neural network which is able to reduce computational burden while considering nonholonomic constraints as well as collision avoidance. Specifically, we suggest a learning method with an efficient adaptive sampling for training dataset for nonholonomic systems. Since the final configuration of the nonholonomic system depends on a sequence of control inputs and intermediate configurations, it requires a considerable number of data samples for training networks. Moreover, it can be a NP-hard problem to find the optimal path if the nonholonomic systems consider arbitrary polygonal obstacles in workspace \cite{reif1998complexity}.

Although neural network approaches based on uniform sampling dataset can learn \ctog{} of configuration space for systems without constraints, learning for nonholonomic systems with the uniform dtaset misleads wrong convergence due to considerable discontinuity of gradient of cost-values. The network trained with the uniform dataset degrade performance of planning for nonholonomic systems.
      
Most previous neural network approaches generate dataset from traditional planners such as RRT* \cite{ichter2018learning,qureshi2018motion,johnson2020dynamically,molina2020learn,ichter2020learned}.  Due to nonholonomic constraints, sometimes there is no control action which connect between two neighbor configuration states and it makes large change of gradient of cost-to-go. Therefore, uniform sampling in configuration space is not able capture features of nonholonomic constraints. Moreover, we consider collision avoidance in the continuous control and state spaces, we need an approach for efficient and effective sampling method.


For the trajectory generation, there is no analytical solution to generate the optimal trajectory while avoiding obstacles although Dubins and Reeds-Shepp curves are optimal in open space. Sampling based methods such as RRTs require intensive collision checks or iterative value computations with satisfying nonholonomic constraints. We also suggest a trajectory generation based on predicted \ctog{} by the trained network.

Compared to previous approach for learning of cost-to-go for motion planning \cite{huh2020cost} with uniform samples from \ctog{} in various workspace, this paper handles nonholonomic constraints additionally and focus on improvement performance of learning with adaptive sampling according to gradient of cost-values and characteristics of dataset. 
    
    

\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figs/main_figure3.png}
\caption{System Overview. Nonholonomic \ctog{} function network is trained to encode an input workspace and to output a cost-to-go function represented by a neural network. The trajectory is generated by choosing a sequence of control as decreasing the cost values.
\label{fig:overview_flowchart}}
%\vspace{-3mm}
\end{figure}

In summary, the core contributions of the paper are 1)~learning approach for cost-to-go estimation of nonholonomic system based on a neural network for various given workspace; 2) efficient adaptive method based on diversity of gradient of cost values and characteristic of non-holonomic system; 3) demonstration of considerable performance improvement compared to traditional approaches.





